A Probabilistic Approach for Demand-Aware Ride-Sharing Optimization

Ride-sharing is a modern urban-mobility paradigm with tremendous potential in reducing congestion and pollution. Demand-aware design is a promising avenue for addressing a critical challenge in ride-sharing systems, namely joint optimization of request-vehicle assignment and routing for a fleet of vehicles. In this paper, we develop a probabilistic demand-aware framework to tackle the challenge. We focus on maximizing the expected number of passenger pickups, given the probability distributions of future demands. The key idea of our approach is to assign requests to vehicles in a probabilistic manner. It differentiates our work from existing ones and allows us to explore a richer design space to tackle the request-vehicle assignment puzzle with a performance guarantee but still keeping the final solution practically implementable. The optimization problem is non-convex, combinatorial, and NP-hard in nature. As a key contribution, we explore the problem structure and propose an elegant approximation of the objective function to develop a dual-subgradient heuristic. We characterize a condition under which the heuristic generates a $\left(1-1/e\right)$ approximation solution. Our solution is simple and scalable, amendable for practical implementation. Results of numerical experiments based on real-world traces in Manhattan show that, as compared to a conventional demand-oblivious scheme, our demand-aware solution improves the passenger pickups by up to 46%. The results also show that joint optimization at the fleet level leads to 19% more pickups than that by separate optimizations at individual vehicles.

==> backup.tex <==
\subsubsection{A Dual Sub-Gradient based Algorithm}

We develop a heuristic dual sub-gradient based algorithm to solve
$TEF2$, named $ALG$. $ALG$ iteratively distributes price of probability
 to each driver and runs a longest path algorithm to derive a route.


\paragraph{The Dual of Problem TEF2}

We relax the constrains (\ref{eq:TEF2_cons1}),(\ref{eq:TEF2_cons2})
to the objective function by introducing Lagrangian dual variables
$\lambda\triangleq[\lambda_{i}]_{i\in[N]}\geq0$, $\mu\triangleq[\mu_{\bar{v},u,k}]_{\bar{v}\in\mathcal{V}^{[\tau]},u\in\mathcal{V},k\in\mathcal{K}}\geq0$
for them respectively, and obtain the following Lagrangian function,
\begin{align*}
 & L\left(x,y,\lambda,\mu\right)\\
= & \sum_{i=1}^{N}\left\{ \sum_{\bar{v}\in\mathcal{V}^{[\tau]}}\left[x_{i,\bar{v}}\left(1-\lambda_{i}\right)\sum_{u\in\mathcal{V}}\sum_{k\in\mathcal{K}}y_{i,\bar{v},u,k}\right]+\lambda_{i}\right\} \\
 & -\sum_{\bar{v}\in\mathcal{V}^{[\tau]}}\sum_{u\in\mathcal{V}}\sum_{k\in\mathcal{K}}\left[\mu_{\bar{v},u,k}\left(\sum_{i=1}^{N}x_{i,\bar{v}}y_{i,\bar{v},u,k}-k\cdot p_{\bar{v},u,k}\right)\right],
\end{align*}
where $x\triangleq[\mathbf{x}_{i}]_{i\in[N]}$, $y\triangleq[y_{i,\bar{v},u,k}]_{i\in[N],\bar{v}\in\mathcal{V}^{[\tau]},u\in\mathcal{V},k\in\mathcal{K}}$
for sake of simplicity. By rearrange the order of the summation and
some combination, we obtain,

\[
\begin{split}L= & \sum_{i=1}^{N}\sum_{\bar{v}\in\mathcal{V}^{[\tau]}}[x_{i,\bar{v}}\sum_{u\in\mathcal{V}}\sum_{k\in\mathcal{K}}(1-\lambda_{i}-\mu_{\bar{v},u,k})y_{i,\bar{v},u,k}]\\
 & +\sum_{i=1}^{N}\lambda_{i}+\sum_{\bar{v}\in\mathcal{V}^{[\tau]}}\sum_{u\in\mathcal{V}}\sum_{k\in\mathcal{K}}\mu_{\bar{v},u,k}\cdot k\cdot p_{\bar{v},u,k}\\
\overset{(a)}{=} & \sum_{i=1}^{N}\sum_{\bar{v}\in\mathcal{V}^{[\tau]}}(x_{i,\bar{v}}w_{i,\bar{v}})+l_{2}(\mathbf{\lambda},\mu)
\end{split}
\]
For $(a)$, to simplify the expression, we denote $l_{2}(\mathbf{\lambda},\mu)=\sum_{i=1}^{N}\lambda_{i}+\sum_{\bar{v}\in\mathcal{V}^{[\tau]}}\sum_{u\in\mathcal{V}}\sum_{k\in\mathcal{K}}\mu_{\bar{v},u,k}\cdot k\cdot p_{\bar{v},u,k}$
and $w_{i,\bar{v}}=\sum_{u\in\mathcal{V}}\sum_{k\in\mathcal{K}}(1-\lambda_{i}-\mu_{\bar{v},u,k})y_{i,\bar{v},u,k}$
. Then the dual function

\begin{eqnarray*}
D(\lambda,\mu) & = & \max_{x,y}L(x,y,\lambda,\mu)\\
 & = & \max_{x,y}\sum_{i=1}^{N}\sum_{\bar{v}\in\mathcal{V}^{[\tau]}}(x_{i,\bar{v}}w_{i,\bar{v}})+l_{2}(\mathbf{\lambda},\mu)\\
 &  & \max_{x}\sum_{i=1}^{N}\sum_{\bar{v}\in\mathcal{V}^{[\tau]}}x_{i,\bar{v}}\max_{y}w_{i,\bar{v}}+l_{2}(\mathbf{\lambda},\mu)
\end{eqnarray*}
In particular, $\max_{y}w_{i,\bar{v}}$ is

\begin{eqnarray*}
\max &  & \sum_{u\in\mathcal{V}}\sum_{k\in\mathcal{K}}(1-\lambda_{i}-\mu_{\bar{v},u,k})y_{i,\bar{v},u,k}\\
s.t &  & 0\leq y_{i,\bar{v},u,k}\leq p_{\bar{v},u,k}\times\mathit{z_{i,\bar{v},u}}.
\end{eqnarray*}
The problem is linear and its optimal solution is

\[
y_{i,\bar{v},u,k}^{*}=\begin{cases}
p_{\bar{v},u,k}\times\mathit{z_{i,\bar{v},u}} & \lambda_{i}+\mu_{\bar{v},u,k}\leq1\\
0, & o.w.
\end{cases}.
\]
We denote $w_{i,\bar{v}}^{*}=\max_{y}w_{i,\bar{v}}$, then 

\begin{eqnarray*}
D(\lambda,\mu) & = & \max_{x}\sum_{i=1}^{N}\sum_{\bar{v}\in\mathcal{V}^{[\tau]}}x_{i,\bar{v}}w_{i,\bar{v}}^{*}+l_{2}(\mathbf{\lambda},\mu)\\
 & = & \sum_{i=1}^{N}\max_{\mathbf{x}_{i}}\sum_{\bar{v}\in\mathcal{V}^{[\tau]}}x_{i,\bar{v}}w_{i,\bar{v}}^{*}+l_{2}(\mathbf{\lambda},\mu)\\
 & \overset{(a)}{=} & \sum_{i=1}^{N}\sum_{\bar{v}\in\mathcal{V}^{[\tau]}}x_{i,\bar{v}}^{*}w_{i,\bar{v}}^{*}+l_{2}(\mathbf{\lambda},\mu)
\end{eqnarray*}
, where $(a)$ is by denoting $[x_{i,\bar{v}}^{*}]_{\bar{v}}=\arg\max_{\mathbf{x}_{i}}\sum x_{i,\bar{v}}$.
To compute $D(\lambda,\mu)$ is equivalent to computed $N$ longest
route ($\triangleq R_{i}^{*}$) for each driver over $G^{[\tau]}$
with weigh $w_{i,\bar{v}}$ for each node $\bar{v}\in\mathcal{V}^{[\tau]}$. 

\paragraph{The ALG}

We further define

\begin{equation}
\gamma_{i}(\lambda,\mu)\triangleq\sum_{\bar{v}\in\mathcal{V}^{[\tau]}}(x_{i,\bar{v}}^{*}\sum_{u\in\mathcal{V}}\sum_{k\in\mathcal{K}}y_{i,\bar{v},u,k}^{*}),\label{eq:gamma}
\end{equation}

\begin{equation}
\eta_{\bar{v},u,k}(\lambda,\mu)\triangleq\sum_{i=1}^{N}x_{i,\bar{v}}^{*}y_{i,\bar{v},u,k}^{*}.\label{eq:eta}
\end{equation}
We first introduce a set of complementary-slackness-like conditions
for $\lambda$ and $\mu$. If the conditions hold, we can derive an
optimal solution to $TEF2$. 
\begin{thm}
\label{thm:optimality} Suppose the dual variables $\lambda$,$\mu$
and ${\gamma_{i}(\lambda,\mu),\forall i\in[N]}$ computed in \ref{eq:gamma}
and $\eta_{\bar{v},u,k}(\lambda,\mu),\forall\bar{v}\in\mathcal{V}^{[tau]},u\in\mathcal{V},k\in\mathcal{K}$
computed in \ref{eq:eta} satisfy that
\begin{equation}
[\gamma_{i}-1]_{\lambda_{i}}^{+}=0,\forall i\in[N],\label{eq:opt1}
\end{equation}
\begin{equation}
\begin{split}[\eta_{\bar{v},u,k}-k\cdot p_{\bar{v},u,k}]_{\mu_{\bar{v},u,k}}^{+} & \forall\bar{v}\in\mathcal{V}^{[tau]},u\in\mathcal{V},k\in\mathcal{K}\end{split}
,\label{eq:opt2}
\end{equation}
where function $[f]_{g}^{+}$is defined as

\[
[f]_{g}^{+}=\begin{cases}
f & g>0\\
\max(f,0) & o.w.
\end{cases}.
\]
Then each $x^{*}$ and \textup{$y^{*}$, }specifying routes for drivers
and probabilistic allocation, is the optimal solution to $TEF2$.
\end{thm}
\begin{proof}
Refer to ....
\end{proof}
%
Our proposed $ALG$, showed in Algorithm \ref{alg:dual}, iteratively
update dual variables towards satisfying the optimal conditions (\ref{eq:opt1}),
(\ref{eq:opt2}):

\[
\dot{\lambda}_{i}=\phi(\lambda_{i})[\gamma_{i}-1]_{\lambda_{i}}^{+},
\]

\[
\dot{\mu}_{\bar{v},u,k}=\phi(\mu_{\bar{v},u,k})[\eta_{\bar{v},u,k}-k\cdot p_{\bar{v},u,k}]_{\mu_{\bar{v},u,k}}^{+}
\]

\begin{algorithm}
\caption{\label{alg:dual}}
\end{algorithm}

 We now consider the following problem: 

\begin{eqnarray}
TEF: & \max & \sum_{i=1}^{N}\min\{1,\sum_{j=1}^{n_{i}}\sum_{u\in\mathcal{V}}\sum_{k\in\mathcal{K}}y_{i,\bar{v},u,k}\}\label{eq:approx-1}\\
 & s.t. & \sum_{i=1}^{N}y_{i,\bar{v},u,k}\leq k\cdot p_{\bar{v},u,k},\\
 &  & 0\leq y_{i,\bar{v},u,k}\leq p_{\bar{v},u,k}.\\
 &  & y_{i,\bar{v},u,k}\leq\mathit{z_{i,\bar{v},u}}\\
 &  & R_{i}^{[\tau]}\in\mathcal{R}_{i}^{[\tau]}\nonumber 
\end{eqnarray}

, in the above formulation, $y_{i,\bar{v},u,k},p_{\bar{v},u,k},\mathit{z_{i,\bar{v},u}},y_{i,\bar{v}}$
correspond to $y_{i,v,u,k}^{t},p_{v,u,k}^{t},\mathit{z_{i,v,u}^{t}},y_{i,v}^{t}$
in (\ref{eq:stage1}),(\ref{eq:approx}).

The relation between and is described by the following theorem,
\begin{thm}
Problem $TEF$ is equivalent to (\ref{eq:approx}).
\end{thm}
\begin{proof}
. k
\end{proof}
%
. . We now introduce a node based equivalent formulation to $TEF$. 

To tackle the hard delay constrains, we introduce an
alternative formulation based on a time-expanded graph. In our work,
the time-expanded graph is defined as as follows.
\begin{defn}
Given $\tau=\max\{\Delta_{s_{i},d_{i}}^{max}\}$ and $G=(\mathcal{V},\mathcal{E})$,
the time-expanded graph $G^{[\tau]}=(\mathcal{V}^{[\tau]},\mathcal{E}^{[\tau]})$
contains $\tau\times|\mathcal{V}|$ nodes, each node is labeled as
$v^{t}$ for all $v\in\mathcal{V},t\in[1,\tau]$.  The edge set $\mathcal{E}^{[\tau]}$
is constructed as follows: 1)For each edge $e=(u,v)\in\mathcal{E}$
with travel delay $\delta_{u,v}$, for each $t\in[1,\tau-\delta_{u,v}]$,
there exists an edge $e^{t}\in\mathcal{E}^{[\tau]}$ from $u^{t}$
to $v^{t+\delta_{u,v}}$. Note that there is no travel delay associated
with $e^{t}$; 2)For each node $u\in\mathcal{V}$, $t\in[1,t-1]$,
there exists an edge in $\mathcal{E}^{t}$ from $u^{t}$ to $u^{t+1}$. 
\end{defn}
For any node $v^t\in \mathcal{V}^{[\tau]}$, it is associated with the probabilities $[p_{v,u,k}^{t}]_{u\in\mathcal{V},k\in[k]}$. Let $\mathcal{R}_{i}^{[\tau]}$ be the set of
all routes that start from $s_{i}^{0}$ to $d_{i}^{\tau_{i}}$ and
a route in $\mathcal{R}_{i}^{[\tau]}$ is denoted as
\[r_{i}^{[\tau]}=(s_{i}^{0},\bar{v}_{i,1},\bar{v}_{i,2},\cdots\cdots,\bar{v}_{i,n_{i}},d_{i}^{\tau_{i}})\]
, where $\tau_{i}=\Delta_{s_{i},d_{i}}^{max}$
and $n_{i}$ is the
number of intermediate nodes. Then the time expanded formulation is: 

\begin{eqnarray}
\mbox{\textbf{MP-T}}: & \max & \sum_{i=1}^{N}f_{i}\left(\mathbf{y_{i}},r_{i}\right)\label{Prob_MP:obj}\\
 & \mbox{var.} & \left[\boldsymbol{y}_{i},1\leq i\leq N\right]\in\mathcal{Y},\;r_{i}^{[\tau]}\in\mathcal{R}_{i}^{[\tau]},\;1\leq i\leq N,\nonumber 
\end{eqnarray}
$y_{i,v,u,k}^{t}$, $p_{v,u,k}^{t}$, $\mathit{z_{i,v,u}^{t}}$, $y_{i,v}^{t}$ are with the same meaning as in problem \textbf{MP}, and associated with node $v^t\in\mathcal{V}^{[\tau]}$ in problem \textbf{MP-T}. In the following discussion, we focus on the problem \textbf{MP-T}.

\begin{eqnarray}
TEF3 & \max & \sum_{i=1}^{N}\sum_{\bar{v}\in\mathcal{V}^{[\tau]}}(x_{i,\bar{v}}\sum_{u\in\mathcal{V}}\sum_{k\in\mathcal{K}}y_{i,\bar{v},u,k})\label{eq:approx-1-1-1}\\
 & s.t. & \sum_{\bar{v}\in\mathcal{V}^{[\tau]}}(x_{i,\bar{v}}\sum_{u\in\mathcal{V}}\sum_{k\in\mathcal{K}}y_{i,\bar{v},u,k})\leq1\label{eq:TEF2_cons1-1}\\
 &  & \sum_{i=1}^{N}x_{i,\bar{v}}y_{i,\bar{v},u,k}\leq k\cdot p_{\bar{v},u,k},\label{eq:TEF2_cons2-1}\\
 &  & 0\leq x_{i,\bar{v}}y_{i,\bar{v},u,k}\leq x_{i,\bar{v}}\times p_{\bar{v},u,k}\times\mathit{z_{i,\bar{v},u}},\label{eq:TEF2_cons3-1}\\
 &  & \mathbf{\mathbf{x}}_{i}\in\mathcal{X}_{i}\nonumber 
\end{eqnarray}

and we claim the $TEF3$ is equivalent to $TEF2$. (The proof will
be added.).

We 
\iffalse
\subsection{Problem Formulation\label{ssec:formulation}}

The joint (probabilistic) request-vehicle assignment and vehicle routing
problem can then be formulated as follows:
\begin{eqnarray}
\mbox{\textbf{MP}}: & \max & \sum_{i=1}^{N}f_{i}\left(\mathbf{y_{i}},r_{i}\right)\label{Prob_MP:obj}\\
 & \mbox{var.} & \left[\boldsymbol{y}_{i},1\leq i\leq N\right]\in\mathcal{Y},\;r_{i}\in\mathcal{R}_{i}^{[\tau]},\;1\leq i\leq N,\nonumber 
\end{eqnarray}
where $\mathcal{R}_{i}^{[\tau]}$ is the set of all routes that start from $s_{i}^{0}$ to $d_{i}^{\tau_{i}}$ on $G^{[\tau]}$, (i.e., following the route, the driver will arrive at node $d_i$ before $\tau_i$  
and $\mathcal{Y}$ is the feasible set described by
a set of linear inequalities in (\ref{cons:proballocation2}) - (\ref{cons:proballocation1}). 

Problem \textbf{MP} {is challenging to solve as it} involves a non-convex objective function and a
combinatorial feasible set for the routes $r_{i}$, $1\leq i\leq N$.
% It is a challenging problem as suggested by the following proposition. 


\subsection{Discussions on the Hardness\label{ssec:hardness}}
\com{Help resolving issues related to Prop. 4 and 8.}

We formulate the problem under the time-expanded graph. A possible concern could be the exponential increment of the expression. More specifically, . Namely, the 


\begin{mdframed}[skipabove=10pt, skipbelow=10pt, roundcorner=10pt, linewidth=0pt, backgroundcolor=gray!10] 
\begin{prop}
\label{prop:MP-is-NP-hard}The problem \textbf{MP }is NP-hard as it
covers the NP-hard single-vehicle demand-aware routing problem in \cite{QiulinRideSharingRouting17}
as a special case. 
\end{prop}
\end{mdframed}
%
\fi
\section{NP-hardness}
How to presenting the NP-harness problem here? A problem is that we formulation the problem based on a time expanded graph whose input size is already polynomial in the value $T$!!!

\section{Time-expanded Graph}
The problem that our explained time-expanded graph is actually not the one will adapt! We can not create an edge from $v^t$ to $v^{t+1}$. 
